A mixed-integer approximation of robust optimization problems with mixed-integer adjustments

In the present article we propose a mixed-integer approximation of adjustable-robust optimization (ARO) problems, that have both, continuous and discrete variables on the lowest level. As these trilevel problems are notoriously hard to solve, we restrict ourselves to weakly-connected instances. Our approach allows us to approximate, and in some cases exactly represent, the trilevel problem as a single-level mixed-integer problem. This allows us to leverage the computational efficiency of state-of-the-art mixed-integer programming solvers. We demonstrate the value of this approach by applying it to the optimization of power systems, particularly to the control of smart converters.

==> keywords.tex <==
Mixed-Integer Optimization;
Robust Optimization; %
Adjustable Robustness

==> msc2010.tex <==
%90Cxx, % Mathematical programming
%90C17, %Robustness in mathematical programming
%90C11, %Mixed integer programming
%90-10, %Mathematical modeling or simulation for problems pertaining to operations research and mathematical programming

